Simulator-based explanation and debugging of hazard-triggering events in DNN-based safety-critical systems

When Deep Neural Networks (DNNs) are used in safety-critical systems, engineers should determine the safety risks associated with failures (i.e., erroneous outputs) observed during testing. For DNNs processing images, engineers visually inspect all failure-inducing images to determine common characteristics among them. Such characteristics correspond to hazard-triggering events (e.g., low illumination) that are essential inputs for safety analysis. Though informative, such activity is expensive and error-prone. To support such safety analysis practices, we propose SEDE, a technique that generates readable descriptions for commonalities in failure-inducing, real-world images and improves the DNN through effective retraining. SEDE leverages the availability of simulators, which are commonly used for cyber-physical systems. It relies on genetic algorithms to drive simulators towards the generation of images that are similar to failure-inducing, real-world images in the test set; it then employs rule learning algorithms to derive expressions that capture commonalities in terms of simulator parameter values. The derived expressions are then used to generate additional images to retrain and improve the DNN. With DNNs performing in-car sensing tasks, SEDE successfully characterized hazard-triggering events leading to a DNN accuracy drop. Also, SEDE enabled retraining leading to significant improvements in DNN accuracy, up to 18 percentage points.

==> context.tex <==
% !TEX root =  MAIN.tex
\section{Motivation and Context}
\label{sec:context}


Most of DNNs used in autonomous systems are trained and tested using both images generated by simulators and real-world images. Because of the labelling costs, real-world images are limited and mostly used for testing. Training is mostly based on simulator images, while testing should include a larger proportion of real-world images to ensure that the system is ready to be delivered. In the presence of DNN failures, the failure-inducing images in the test set can be inspected by engineers to improve the DNN. The visual inspection of such images may enable engineers to identify scenarios that are unsafe (i.e., the DNN generates erroneous results), and collect additional related real-world images or configure the simulator to generate them. Given that this is an expensive activity, in this work, we propose a solution to automate the identification and characterization of unsafe scenarios observed in real-world images to enable generating simulator images that present similar triggering events and minimize retraining costs. 



==> tables/RQ1-FLD.tex <==
\begin{table}[t]
\centering
\smaller
\caption{RQ1: Average diversity across RCCs for FLD}
\begin{tabular}{|c|ccc|cccc|}
\hline
\begin{tabular}[c]{@{}c@{}}Time (hrs.)\end{tabular} & 
\multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. diversity (standard deviation) \\across RCCs\end{tabular}} & 
\multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Statistical test\end{tabular}} &
%\hline 
& 
&
&
&
 \multicolumn{2}{c|}{NSGA-II} & \multicolumn{2}{c|}{DeepNSGA-II} & 
 &
\multicolumn{1}{C{1.2cm}|}{\GAAlg} & \multicolumn{1}{C{1.4cm}|}{NSGA-II} &  \multicolumn{1}{C{1.6cm}|}{DeepNSGA-II} & 
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textit{p-value} \\(U-test)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Effect Size \\ ($\hat{A}_{12}$)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textit{p-value} \\(U-test)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Effect Size \\ ($\hat{A}_{12}$)\end{tabular}}
 
\\ \hline

5 & \multicolumn{1}{c|}{0.200 (0.077)} & \multicolumn{1}{c|}{0.137 (0.067)} & \multicolumn{1}{c|}{0.010 (0.045)} & \multicolumn{1}{c|}{4.47e-05} & \multicolumn{1}{c|}{0.765} & \multicolumn{1}{c|}{6.06e-13} & \multicolumn{1}{c|}{0.932} 
\\ \hline
10 & \multicolumn{1}{c|}{0.200 (0.077)} & \multicolumn{1}{c|}{0.028 (0.040)} & \multicolumn{1}{c|}{0.178 (0.061)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.015} & \multicolumn{1}{c|}{0.657} 
\\ \hline
15 & \multicolumn{1}{c|}{0.202 (0.077)} & \multicolumn{1}{c|}{0.012 (0.020)} & \multicolumn{1}{c|}{0.181 (0.063)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.028} & \multicolumn{1}{c|}{0.643} 
\\ \hline
20 & \multicolumn{1}{c|}{0.202 (0.077)} & \multicolumn{1}{c|}{0.005 (0.003)} & \multicolumn{1}{c|}{0.182 (0.063)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.013} & \multicolumn{1}{c|}{0.660} 
\\ \hline
25 & \multicolumn{1}{c|}{0.203 (0.077)} & \multicolumn{1}{c|}{0.005 (0.003)} & \multicolumn{1}{c|}{0.183 (0.064)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.028} & \multicolumn{1}{c|}{0.643} 
\\ \hline
30 & \multicolumn{1}{c|}{0.210 (0.080)} & \multicolumn{1}{c|}{0.004 (0.002)} & \multicolumn{1}{c|}{0.184 (0.064)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.002} & \multicolumn{1}{c|}{0.700} 
\\ \hline
35 & \multicolumn{1}{c|}{0.211 (0.080)} & \multicolumn{1}{c|}{0.006 (0.005)} & \multicolumn{1}{c|}{0.185 (0.065)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.001} & \multicolumn{1}{c|}{0.705} 
\\ \hline
40 & \multicolumn{1}{c|}{0.211 (0.080)} & \multicolumn{1}{c|}{0.004 (0.002)} & \multicolumn{1}{c|}{0.185 (0.065)} & \multicolumn{1}{c|}{4.36e-10} & \multicolumn{1}{c|}{0.905} & \multicolumn{1}{c|}{0.001} & \multicolumn{1}{c|}{0.705} 
\\ \hline
\end{tabular}
\label{tab:rq1_1_fld}
\end{table}

==> tables/RQ1-HPD1.tex <==
\begin{table}[t]
\centering
\smaller
\caption{RQ1: Average diversity across RCCs for HPD-F}
\begin{tabular}{|c|ccc|cccc|}
\hline
\begin{tabular}[c]{@{}c@{}}Time (hrs.)\end{tabular} & 
\multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. diversity (standard deviation) \\across RCCs\end{tabular}} & 
\multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Statistical test\end{tabular}} &
%\hline 
& 
&
&
&
 \multicolumn{2}{c|}{NSGA-II} & \multicolumn{2}{c|}{DeepNSGA-II} & 
 &
\multicolumn{1}{C{1.2cm}|}{\GAAlg} & \multicolumn{1}{C{1.4cm}|}{NSGA-II} &  \multicolumn{1}{C{1.6cm}|}{DeepNSGA-II} & 
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textit{p-value} \\(U-test)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Effect Size \\ ($\hat{A}_{12}$)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textit{p-value} \\(U-test)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Effect Size \\ ($\hat{A}_{12}$)\end{tabular}}
 
\\ \hline
5 & \multicolumn{1}{c|}{2.9e-4 (7.6e-4)} & \multicolumn{1}{c|}{0.0 (0.0)} & \multicolumn{1}{c|}{2.1e-4 (7.8e-4)} & \multicolumn{1}{c|}{0.003} & \multicolumn{1}{c|}{0.600} & \multicolumn{1}{c|}{0.141} & \multicolumn{1}{c|}{0.557} \\ \hline

10 & \multicolumn{1}{c|}{0.009 (0.016)} & \multicolumn{1}{c|}{0.011 (0.019)} & \multicolumn{1}{c|}{0.002 (0.006)} & \multicolumn{1}{c|}{0.739} & \multicolumn{1}{c|}{0.520} & \multicolumn{1}{c|}{0.041} & \multicolumn{1}{c|}{0.639} \\ \hline

15 & \multicolumn{1}{c|}{0.010 (0.013)} & \multicolumn{1}{c|}{0.002 (0.003)} & \multicolumn{1}{c|}{0.006 (0.008)} & \multicolumn{1}{c|}{0.008} & \multicolumn{1}{c|}{0.660} & \multicolumn{1}{c|}{0.275} & \multicolumn{1}{c|}{0.568} \\ \hline

20 & \multicolumn{1}{c|}{0.010 (0.014)} & \multicolumn{1}{c|}{0.002 (0.002)} & \multicolumn{1}{c|}{0.008 (0.010)} & \multicolumn{1}{c|}{5.53e-4} & \multicolumn{1}{c|}{0.715} & \multicolumn{1}{c|}{0.468} & \multicolumn{1}{c|}{0.545} \\ \hline

25 & \multicolumn{1}{c|}{0.011 (0.013)} & \multicolumn{1}{c|}{0.002 (0.002)} & \multicolumn{1}{c|}{0.010 (0.011)} & \multicolumn{1}{c|}{5.45e-05} & \multicolumn{1}{c|}{0.750} & \multicolumn{1}{c|}{0.862} & \multicolumn{1}{c|}{0.511} \\ \hline

30 & \multicolumn{1}{c|}{0.013 (0.014)} & \multicolumn{1}{c|}{0.002 (0.002)} & \multicolumn{1}{c|}{0.011 (0.011)} & \multicolumn{1}{c|}{5.45e-05} & \multicolumn{1}{c|}{0.750} & \multicolumn{1}{c|}{0.862} & \multicolumn{1}{c|}{0.511} \\ \hline

35 & \multicolumn{1}{c|}{0.013 (0.014)} & \multicolumn{1}{c|}{0.002 (0.002)} & \multicolumn{1}{c|}{0.012 (0.011)} & \multicolumn{1}{c|}{6.18e-06} & \multicolumn{1}{c|}{0.780} & \multicolumn{1}{c|}{0.956} & \multicolumn{1}{c|}{0.504} \\ \hline

40 & \multicolumn{1}{c|}{0.014 (0.015)} & \multicolumn{1}{c|}{0.002 (0.003)} & \multicolumn{1}{c|}{0.012 (0.011)} & \multicolumn{1}{c|}{1.31e-05} & \multicolumn{1}{c|}{0.770} & \multicolumn{1}{c|}{0.817} & \multicolumn{1}{c|}{0.515} \\ \hline
\end{tabular}
\label{tab:rq1_1_hpdf}
\end{table}

==> tables/RQ1-HPD2.tex <==
\begin{table}[t]
\centering
\smaller
\caption{RQ1: Average diversity across RCCs for HPD-H}
\begin{tabular}{|c|ccc|cccc|}
\hline
\begin{tabular}[c]{@{}c@{}}Time (hrs.)\end{tabular} & 
\multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. diversity (standard deviation) \\across RCCs\end{tabular}} & 
\multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Statistical test\end{tabular}} &
%\hline 
& 
&
&
&
 \multicolumn{2}{c|}{NSGA-II} & \multicolumn{2}{c|}{DeepNSGA-II} & 
 &
\multicolumn{1}{C{1.2cm}|}{\GAAlg} & \multicolumn{1}{C{1.4cm}|}{NSGA-II} &  \multicolumn{1}{C{1.6cm}|}{DeepNSGA-II} & 
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textit{p-value} \\(U-test)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Effect Size \\ ($\hat{A}_{12}$)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textit{p-value} \\(U-test)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Effect Size \\ ($\hat{A}_{12}$)\end{tabular}}
 
\\ \hline

5 & \multicolumn{1}{c|}{0.022 (0.032)} & \multicolumn{1}{c|}{0.024 (0.050)} & \multicolumn{1}{c|}{0.001 (0.005)} & \multicolumn{1}{c|}{0.055} & \multicolumn{1}{c|}{0.610} & \multicolumn{1}{c|}{2.19e-09} & \multicolumn{1}{c|}{0.827} \\ \hline

10 & \multicolumn{1}{c|}{0.028 (0.039)} & \multicolumn{1}{c|}{0.005 (0.008)} & \multicolumn{1}{c|}{0.012 (0.010)} & \multicolumn{1}{c|}{0.002} & \multicolumn{1}{c|}{0.686} & \multicolumn{1}{c|}{0.843} & \multicolumn{1}{c|}{0.512} \\ \hline

15 & \multicolumn{1}{c|}{0.029 (0.037)} & \multicolumn{1}{c|}{0.001 (0.002)} & \multicolumn{1}{c|}{0.013 (0.010)} & \multicolumn{1}{c|}{6.60e-09} & \multicolumn{1}{c|}{0.855} & \multicolumn{1}{c|}{0.583} & \multicolumn{1}{c|}{0.534} \\ \hline

20 & \multicolumn{1}{c|}{0.028 (0.035)} & \multicolumn{1}{c|}{0.001 (0.001)} & \multicolumn{1}{c|}{0.015 (0.009)} & \multicolumn{1}{c|}{1.98e-10} & \multicolumn{1}{c|}{0.893} & \multicolumn{1}{c|}{0.844} & \multicolumn{1}{c|}{0.488} \\ \hline

25 & \multicolumn{1}{c|}{0.029 (0.036)} & \multicolumn{1}{c|}{0.003 (0.004)} & \multicolumn{1}{c|}{0.017 (0.008)} & \multicolumn{1}{c|}{1.36e-08} & \multicolumn{1}{c|}{0.851} & \multicolumn{1}{c|}{0.716} & \multicolumn{1}{c|}{0.477} \\ \hline

50 & \multicolumn{1}{c|}{0.056 (0.049)} & \multicolumn{1}{c|}{0.002 (0.002)} & \multicolumn{1}{c|}{0.034 (0.035)} & \multicolumn{1}{c|}{2.30e-12} & \multicolumn{1}{c|}{0.934} & \multicolumn{1}{c|}{0.057} & \multicolumn{1}{c|}{0.618} \\ \hline

75 & \multicolumn{1}{c|}{0.072 (0.061)} & \multicolumn{1}{c|}{0.003 (0.002)} & \multicolumn{1}{c|}{0.085 (0.050)} & \multicolumn{1}{c|}{1.20e-13} & \multicolumn{1}{c|}{0.959} & \multicolumn{1}{c|}{0.057} & \multicolumn{1}{c|}{0.382} \\ \hline

100 & \multicolumn{1}{c|}{0.088 (0.063)} & \multicolumn{1}{c|}{0.003 (0.002)} & \multicolumn{1}{c|}{0.107 (0.042)} & \multicolumn{1}{c|}{6.37e-16} & \multicolumn{1}{c|}{1.0} & \multicolumn{1}{c|}{0.083} & \multicolumn{1}{c|}{0.393} \\ \hline

125 & \multicolumn{1}{c|}{0.102 (0.071)} & \multicolumn{1}{c|}{0.003 (0.002)} & \multicolumn{1}{c|}{0.118 (0.042)} & \multicolumn{1}{c|}{6.37e-16} & \multicolumn{1}{c|}{1.0} & \multicolumn{1}{c|}{0.230} & \multicolumn{1}{c|}{0.426} \\ \hline

150 & \multicolumn{1}{c|}{0.120 (0.083)} & \multicolumn{1}{c|}{0.003 (0.003)} & \multicolumn{1}{c|}{0.120 (0.034)} & \multicolumn{1}{c|}{6.37e-16} & \multicolumn{1}{c|}{1.0} & \multicolumn{1}{c|}{0.334} & \multicolumn{1}{c|}{0.440} \\ \hline

175 & \multicolumn{1}{c|}{0.140 (0.095)} & \multicolumn{1}{c|}{0.003 (0.002)} & \multicolumn{1}{c|}{0.130 (0.027)} & \multicolumn{1}{c|}{6.37e-16} & \multicolumn{1}{c|}{1.0} & \multicolumn{1}{c|}{0.351} & \multicolumn{1}{c|}{0.442} \\ \hline

200 & \multicolumn{1}{c|}{0.151 (0.093)} & \multicolumn{1}{c|}{0.003 (0.003)} & \multicolumn{1}{c|}{0.129 (0.023)} & \multicolumn{1}{c|}{6.37e-16} & \multicolumn{1}{c|}{1.0} & \multicolumn{1}{c|}{0.95} & \multicolumn{1}{c|}{0.504} \\ \hline
\end{tabular}
\label{tab:rq1_1_hpdh}
\end{table}

==> tables/inputPART.tex <==
\begin{table*}[tb]
\centering
\caption{Input to PART}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
ID & CameraDirection_X & CameraDirection_Y & CameraDirection_Z & CameraLocation_X & CameraLocation_Y & CameraLocation_Z & LampLocation_X & LampLocation_Y & LampLocation_Z & H_Headpose & V_Headpose & T_Headpose & makeHuman_Model

\\ \hline 
1 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ 
\\ \hline
1 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ 
\\ \hline
1 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$  
\\ \hline
1 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ 
\\ \hline
0 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$  
\\ \hline
0 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ 
\\ \hline
0 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$  
\\ \hline
0 & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ & $0.$ 
\\ \hline 
\end{tabular}
\label{tab:inputPART}
\end{table*}

==> tables/old_RQ5.tex <==
\begin{table*}[t]
\centering
\caption{RQ5: Unsafe set size and the accuracy improvement of \APPR compared to HUDD and random baseline (RBL)}
\begin{tabular}{|c|c|cc|c|c|cc|cc|}
\hline
DNN & Original Model & 
\multicolumn{2}{c|}{Retraining Set Size} & 
RBL  & HUDD  & 
\multicolumn{2}{c|}{\APPR} &
\multicolumn{2}{c|}{Stat. Sig.} 
\\ 
%\hline
& Accuracy  & 
\begin{tabular}[c]{@{}c@{}}Training Set\\ (Sim. + Real)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Unsafe\\ Set\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Accuracy (Gain)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Accuracy (Gain)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Accuracy (Gain)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gain over\\ best baseline\end{tabular} &
p-value & $\hat{A}_{12}$
\\ \hline

FLD & 80.06\% & 
\multicolumn{1}{c|}{150 + 6,000} & \multicolumn{1}{c|}{450} &
77.41\% (\textbf{-2.65\%}) & 79.94\% (\textbf{-0.11\%}) & 
\multicolumn{1}{c|}{86.14\% (\textbf{+6.07\%})} & \multicolumn{1}{c|}{\textbf{+6.19\%}}
& 1e-4 & 1.0
\\ \hline

HPD-F & 51.65\% & 
\multicolumn{1}{c|}{1,075 + 476} & \multicolumn{1}{c|}{350} &
44.33\% (\textbf{-7.32\%}) & 45.80\% (\textbf{-5.85\%}) & 
\multicolumn{1}{c|}{56.15\% (\textbf{+4.50\%})} &  \multicolumn{1}{c|}{\textbf{+10.35\%}} 
& 4e-4 & 0.94
\\ \hline

HPD-H & 51.03\% & 
\multicolumn{1}{c|}{900 + 476} & \multicolumn{1}{c|}{500} &
55.57\% (\textbf{+4.54\%})& 60.65\% (\textbf{+9.62\%}) &
\multicolumn{1}{c|}{69.68\% (\textbf{+18.65\%})} &  \multicolumn{1}{c|}{\textbf{+9.03\%}} 
& 1e-4 & 1.0
\\ \hline

\end{tabular}
\label{tab:rq5}
\end{table*}

==> tables/old_dnns.tex <==
% !TEX root =  ../MAIN.tex
\begin{table*}[t]
\caption{Case Study Systems}
\footnotesize
\begin{tabular}{|@{\hspace{1pt}}p{9mm}|@{\hspace{1pt}}p{13mm}|p{12mm}|p{17mm}|p{15mm}|p{6mm}|p{17mm}|p{22mm}|p{20mm}|p{6mm}|}
\hline
DNN &  \multicolumn{2}{c|}{Data Source}& \multicolumn{3}{c|}{Simulator-based Training} & \multicolumn{4}{c|}{Fine-tuning} \\
& Simulator & Real-world & Training Set Size (Accuracy \%) & Test Set Size (Accuracy \%) & Epochs & Training Set Size (Accuracy \%) & Simulator-based Test Set Size (Accuracy \%) & Real-world Test Set Size (Accuracy \%) & Epochs\\
\hline
FLD & IEE-Faces & IEE & 16,000 (99.92\%) & 2,750 (44.41\%) & 10 & 9,000 (95.44\%) 
& 2,825 (43.22\%) %(2,825)  
& 1,000 (80.06\%) %(1,000)
&  50  \\
HPD-F & IEE-Faces & BIWI & 21,500 (91.20\%) & 2,750 (85.43\%) & 18 & 21,976 (95.35\%) 
& 2,200 (87.10\%) %(2,200)  
& 500 (51.65\%) %(500)
& 9  \\
HPD-H & IEE-Humans & BIWI & 15,400 (85.38\%) & 3,000 (80.21\%) & 25 & 18,476 (90.23\%) 
& 2,750 (85.23\%) %(2,750) 
& 500 (51.03\%) %(500) 
& 28 \\
\hline
\end{tabular}

\label{tab:dnns}
\end{table*}%

